FastPoseCNN: Real-Time Monocular Category-Level Pose and Size Estimation Framework

The primary focus of this paper is the development of a framework for pose and size estimation of unseen objects given a single RGB image - all in real-time. In 2019, the first category-level pose and size estimation framework was proposed alongside two novel datasets called CAMERA and REAL. However, current methodologies are restricted from practical use because of its long inference time (2-4 fps). Their approach's inference had significant delays because they used the computationally expensive MaskedRCNN framework and Umeyama algorithm. To optimize our method and yield real-time results, our framework uses the efficient ResNet-FPN framework alongside decoupling the translation, rotation, and size regression problem by using distinct decoders. Moreover, our methodology performs pose and size estimation in a global context - i.e., estimating the involved parameters of all captured objects in the image all at once. We perform extensive testing to fully compare the performance in terms of precision and speed to demonstrate the capability of our method.

==> Figures/background/mathematical_framework.tex <==

\newcommand{\SCALE}{0.75}

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-\SCALE,xscale=\SCALE,every node/.style={scale=1.1*\SCALE}]
%uncomment if require: \path (0,384); %set diagram left start at 0, and has height of 384

%Straight Lines [id:da9174814735619918] 
\draw [color={rgb, 255:red, 177; green, 177; blue, 177 }  ,draw opacity=1 ]   (239.11,325.06) -- (239.11,380.11) ;
%Straight Lines [id:da10444016560016967] 
\draw    (175.94,129.78) -- (312.53,222.66) ;
%Image [id:dp5296325783563776] 
\draw (293.67,54.25) node  {\includegraphics[width=47.59pt,height=47.59pt]{Figures/background/images/mathematical_framework/laptop.PNG}};
%Straight Lines [id:da14584800642464768] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (297.53,48.25) -- (360.82,178.36) ;
%Straight Lines [id:da5158148912123679] 
\draw    (297.53,128.34) -- (501.93,267.65) ;
%Image [id:dp1763408378823499] 
\draw (418.08,295.44) node  {\includegraphics[width=30.33pt,height=19.72pt]{Figures/background/images/mathematical_framework/camera.PNG}};
%Straight Lines [id:da5077912223359735] 
\draw    (361.74,312.41) -- (565.7,247.15) ;
%Straight Lines [id:da30189676419401357] 
\draw    (180.82,165.75) -- (384.77,100.48) ;
%Straight Lines [id:da9708578844569418] 
\draw    (418.35,149.1) -- (418.35,328.48) ;
%Shape: Parallelogram [id:dp7449727065679421] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.54 ] (385.95,120.18) -- (385.95,278.3) -- (239.11,325.06) -- (239.11,166.93) -- cycle ;
%Straight Lines [id:da03860849061983451] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (360.82,178.36) -- (417.9,293.92) ;
%Straight Lines [id:da4952380278690536] 
\draw    (239.21,245.67) -- (386.05,199.26) ;
%Straight Lines [id:da3895823949879542] 
\draw    (312.53,143.49) -- (312.53,301.82) ;
%Straight Lines [id:da42647590861166096] 
\draw    (239.11,166.92) -- (239.11,341.17) ;
\draw [shift={(239.11,344.17)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da32063815200338475] 
\draw    (239.11,166.92) -- (411.78,111.7) ;
\draw [shift={(414.64,110.78)}, rotate = 522.27] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da8547472764556476] 
\draw    (297.53,48.25) -- (297.53,128.34) ;
%Shape: Circle [id:dp19598461831397773] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (358.73,178.36) .. controls (358.73,177.21) and (359.66,176.28) .. (360.82,176.28) .. controls (361.97,176.28) and (362.9,177.21) .. (362.9,178.36) .. controls (362.9,179.52) and (361.97,180.45) .. (360.82,180.45) .. controls (359.66,180.45) and (358.73,179.52) .. (358.73,178.36) -- cycle ;
%Straight Lines [id:da4208842469399443] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ]   (418.55,294.43) -- (450.03,284.01) ;
\draw [shift={(452.88,283.06)}, rotate = 521.69] [fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da40114646901777995] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ]   (418.55,294.43) -- (418.44,322.67) ;
\draw [shift={(418.43,325.67)}, rotate = 270.21] [fill={rgb, 255:red, 0; green, 0; blue, 255 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da5024557685057458] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ]   (297.53,48.25) -- (274.92,44.95) ;
\draw [shift={(271.95,44.52)}, rotate = 368.28999999999996] [fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da6638840226912652] 
\draw [color={rgb, 255:red, 0; green, 255; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ]   (297.53,48.25) -- (297.51,26.44) ;
\draw [shift={(297.5,23.44)}, rotate = 449.92] [fill={rgb, 255:red, 0; green, 255; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da3012493123715465] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ]   (297.53,48.25) -- (286.49,59.49) ;
\draw [shift={(284.39,61.63)}, rotate = 314.48] [fill={rgb, 255:red, 0; green, 0; blue, 255 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Shape: Polygon [id:ds010188696533914854] 
\draw  [color={rgb, 255:red, 0; green, 255; blue, 255 }  ,draw opacity=1 ] (260.76,71.51) -- (260.76,31.93) -- (282.51,24.08) -- (282.21,55.2) -- cycle ;
%Shape: Polygon [id:ds29369325895569687] 
\draw  [color={rgb, 255:red, 0; green, 255; blue, 255 }  ,draw opacity=1 ] (313.63,84.51) -- (313.94,37.97) -- (326.63,25.89) -- (323.6,63.96) -- cycle ;
%Shape: Polygon [id:ds17415657683094565] 
\draw  [color={rgb, 255:red, 0; green, 255; blue, 255 }  ,draw opacity=1 ] (313.94,37.97) -- (260.76,31.93) -- (282.51,24.08) -- (326.63,25.89) -- cycle ;
%Shape: Polygon [id:ds3419585411375463] 
\draw  [color={rgb, 255:red, 0; green, 255; blue, 255 }  ,draw opacity=1 ] (260.76,71.51) -- (260.76,31.93) -- (313.94,37.97) -- (313.63,84.51) -- cycle ;
%Straight Lines [id:da7192656797744814] 
\draw [color={rgb, 255:red, 0; green, 255; blue, 255 }  ,draw opacity=1 ]   (320.38,63) -- (323.6,63.96) ;
%Shape: Circle [id:dp841720752107602] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 255 }  ,fill opacity=1 ] (310.44,222.66) .. controls (310.44,221.5) and (311.38,220.57) .. (312.53,220.57) .. controls (313.68,220.57) and (314.62,221.5) .. (314.62,222.66) .. controls (314.62,223.81) and (313.68,224.74) .. (312.53,224.74) .. controls (311.38,224.74) and (310.44,223.81) .. (310.44,222.66) -- cycle ;
%Straight Lines [id:da2894664374083238] 
\draw    (312.53,222.66) -- (449.13,315.46) ;
%Straight Lines [id:da9274686702086969] 
\draw [color={rgb, 255:red, 177; green, 177; blue, 177 }  ,draw opacity=1 ]   (182,185.44) -- (239.11,166.92) ;
%Straight Lines [id:da3323269488606435] 
\draw [color={rgb, 255:red, 177; green, 177; blue, 177 }  ,draw opacity=1 ]   (182,343.59) -- (239.11,325.06) ;
%Straight Lines [id:da30816439361783354] 
\draw [color={rgb, 255:red, 177; green, 177; blue, 177 }  ,draw opacity=1 ]   (385.95,278.3) -- (385.95,333.35) ;
%Straight Lines [id:da18608618477531147] 
\draw [color={rgb, 255:red, 0; green, 255; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ]   (418.55,294.43) -- (393.73,277.79) ;
\draw [shift={(391.24,276.11)}, rotate = 393.85] [fill={rgb, 255:red, 0; green, 255; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da3687280127900756] 
\draw    (192.5,185.44) -- (192.5,337.59) ;
\draw [shift={(192.5,340.59)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
\draw [shift={(192.5,182.44)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da6532238390619804] 
\draw    (383.1,325.76) -- (241.97,370.7) ;
\draw [shift={(239.11,371.61)}, rotate = 342.34000000000003] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
\draw [shift={(385.95,324.85)}, rotate = 162.34] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Image [id:dp031506577958771986] 
\draw (403.53,41.64) node  {\includegraphics[width=25pt,height=15.44pt]{Figures/background/images/mathematical_framework/laptop2.PNG}};
%Image [id:dp06320592397087443] 
\draw (526.7,54.67) node  {\includegraphics[width=43.26pt,height=40.2pt]{Figures/background/images/mathematical_framework/laptop3.PNG}};
%Straight Lines [id:da33795874207887233] 
\draw    (424.11,41.36) -- (499.1,41.36) ;
\draw [shift={(502.1,41.36)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da8778910640093129] 
\draw    (494.43,70.02) -- (336.44,69.68) ;
\draw [shift={(333.44,69.67)}, rotate = 360.12] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;

% Text Node
\draw (161.09,120.95) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$z$};
% Text Node
\draw (452.5,285.14) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$x_{c}$};
% Text Node
\draw (398.74,310.63) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$y_{c}$};
% Text Node
\draw (380.05,274.27) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$z_{c}$};
% Text Node
\draw (418.12,258.7) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\{C\}$};
% Text Node
\draw (243.27,333.33) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$v$};
% Text Node
\draw (420.28,105.14) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$u$};
% Text Node
\draw (195.43,246.72) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$H$};
% Text Node
\draw (308.93,323.22) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$W$};
% Text Node
\draw (238.72,5.25) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\{O\}$};
% Text Node
\draw (292.55,3.27) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$z_{o}$};
% Text Node
\draw (240.38,30.05) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$x_{o}$};
% Text Node
\draw (263.38,80.05) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$y_{o}$};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (323,156.88) -- (378,156.88) -- (378,170.88) -- (323,170.88) -- cycle  ;
\draw (326,160.88) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {Centroid (x, y)};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (305.67,95.55) -- (342.67,95.55) -- (342.67,109.55) -- (305.67,109.55) -- cycle  ;
\draw (308.67,99.55) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {depth (z)};
% Text Node
\draw (245.15,315.03) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-341.65] [align=left] {image plane};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (438.67,35.05) -- (481.67,35.05) -- (481.67,49.05) -- (438.67,49.05) -- cycle  ;
\draw (441.67,39.05) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {size (w,h,l)};
% Text Node
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ]  (400.67,63.71) -- (444.67,63.71) -- (444.67,77.71) -- (400.67,77.71) -- cycle  ;
\draw (403.67,67.71) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {rotation (q)};


\end{tikzpicture}


==> Figures/literature_review/pose_estimation_method_categories.tex <==
\newcommand{\SCALE}{0.6}

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-\SCALE,xscale=\SCALE,every node/.style={scale=1.1*\SCALE}]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp04536847876474348] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (294.5,39.67) -- (406.25,39.67) -- (406.25,58.75) -- (294.5,58.75) -- cycle ;
%Shape: Rectangle [id:dp4507391002407566] 
\draw   (97.9,86.67) -- (209.9,86.67) -- (209.9,200) -- (97.9,200) -- cycle ;
%Shape: Rectangle [id:dp8951763520158429] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (97.9,86.67) -- (209.9,86.67) -- (209.9,105.33) -- (97.9,105.33) -- cycle ;
%Shape: Rectangle [id:dp2272276250216252] 
\draw   (228,86.67) -- (340,86.67) -- (340,200) -- (228,200) -- cycle ;
%Shape: Rectangle [id:dp28741180917284814] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (229,86.67) -- (340,86.67) -- (340,105.33) -- (228,105.33) -- cycle ;
%Shape: Rectangle [id:dp7905242669227472] 
\draw   (357.5,86.67) -- (469.5,86.67) -- (469.5,200) -- (357.5,200) -- cycle ;
%Shape: Rectangle [id:dp5930490440168175] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (357.5,86.67) -- (469.5,86.67) -- (469.5,105.33) -- (357.5,105.33) -- cycle ;
%Shape: Rectangle [id:dp3178789979587011] 
\draw   (488,86.17) -- (600,86.17) -- (600,199.5) -- (488,199.5) -- cycle ;
%Shape: Rectangle [id:dp6313701032326051] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (488,86.17) -- (600,86.17) -- (600,104.83) -- (488,104.83) -- cycle ;
%Straight Lines [id:da10157896717796366] 
\draw    (350.25,70.25) -- (350.25,59.25) ;
%Straight Lines [id:da27213818214292385] 
\draw    (156.25,69.75) -- (546.75,69.75) ;
%Straight Lines [id:da46541648594384055] 
\draw    (156.25,69.75) -- (156.25,83.75) ;
\draw [shift={(156.25,86.75)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da9352144136545226] 
\draw    (285.81,69.86) -- (285.81,83.86) ;
\draw [shift={(285.81,86.86)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da7805914724774567] 
\draw    (416.81,69.86) -- (416.81,83.86) ;
\draw [shift={(416.81,86.86)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da0644942237820918] 
\draw    (545.81,69.86) -- (545.81,83.86) ;
\draw [shift={(545.81,86.86)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;

% Text Node
\draw (153.9,96) node  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{76.16pt}\setlength\topsep{0pt}
{\small RGB Images}
\end{minipage}};
% Text Node
\draw (153.9,152.67) node   [align=left] {\begin{minipage}[lt]{76.16pt}\setlength\topsep{0pt}
{\tiny PoseCNN \cite{Xiang2017_PoseCNN}}\\{\tiny DPOD \cite{Zakharov2019_DPOD}}\\{\tiny PVNet \cite{Pent2018_PVNet}}\\{\tiny DOPE \cite{Tremblay2018_DOPE}}\\{\tiny BB8 \cite{Rad2017_BB8}}
\end{minipage}};
% Text Node
\draw (350.38,49.21) node  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{75.99pt}\setlength\topsep{0pt}
{\small Input Data Types}
\end{minipage}};
% Text Node
\draw (284,96) node  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{76.16pt}\setlength\topsep{0pt}
{\small RGBD Images}
\end{minipage}};
% Text Node
\draw (284,152.67) node   [align=left] {\begin{minipage}[lt]{76.16pt}\setlength\topsep{0pt}
{\tiny NOCS \cite{Wang2019_NOCS}}\\{\tiny MaskedFusion \cite{Pereira2019_MaskedFusion}}\\{\tiny Brachmann et al. \cite{Brachmann2014_3DObjectCoordinates}}\\{\tiny iPose \cite{Jafari2017_iPose}}\\{\tiny LatentFusion \cite{Park2019_LatentFusion}}
\end{minipage}};
% Text Node
\draw (413.5,96) node  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{76.16pt}\setlength\topsep{0pt}
{\small D Images}
\end{minipage}};
% Text Node
\draw (413.5,152.67) node   [align=left] {\begin{minipage}[lt]{76.16pt}\setlength\topsep{0pt}
{\tiny CLPRDI \cite{Sahin2018_CLPRDI}}\\{\tiny 6OPEDI \cite{Tan2017}}
\end{minipage}};
% Text Node
\draw (544,95.5) node  [color={rgb, 255:red, 254; green, 254; blue, 254 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{76.16pt}\setlength\topsep{0pt}
{\small Point Clouds}
\end{minipage}};
% Text Node
\draw (544,152.17) node   [align=left] {\begin{minipage}[lt]{76.16pt}\setlength\topsep{0pt}
{\tiny W-PoseNet \cite{Xu2019_W-PoseNet}}\\{\tiny DenseFusion \cite{Wang2019_DenseFusion}}\\{\tiny G2L-Net \cite{Chen2020_G2L-Net}}\\{\tiny 6OPRSLPC \cite{Gao2020_PoseRegressionPC}}
\end{minipage}};


\end{tikzpicture}


==> Figures/methodology/data_representation.tex <==
\begin{figure}

\newcommand{\leftTrim}{1cm}
\newcommand{\bottomTrim}{9cm}
\newcommand{\rightTrim}{13cm}
\newcommand{\topTrim}{1cm}

\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.8\linewidth, trim={\leftTrim, \bottomTrim, \rightTrim, \topTrim}, clip]{diagrams/images/data_representation/4-rgb.png}
  \caption{Input RGB image}
  \label{fig:sfig1}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.8\linewidth, trim={\leftTrim, \bottomTrim, \rightTrim, \topTrim}, clip]{diagrams/images/data_representation/4-pred_mask.png}
  \caption{Mask}
  \label{fig:sfig2}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.8\linewidth, trim={\leftTrim, \bottomTrim, \rightTrim, \topTrim}, clip]{diagrams/images/data_representation/4-pred_quat.png}
  \caption{Quaternion}
  \label{fig:sfig2}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.8\linewidth, trim={\leftTrim, \bottomTrim, \rightTrim, \topTrim}, clip]{diagrams/images/data_representation/4-pred_scales.png}
  \caption{Scales}
  \label{fig:sfig2}
\end{subfigure}

\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.8\linewidth, trim={\leftTrim, \bottomTrim, \rightTrim, \topTrim}, clip]{diagrams/images/data_representation/4-pred_z.png}
  \caption{Depth}
  \label{fig:sfig2}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.8\linewidth, trim={\leftTrim, \bottomTrim, \rightTrim, \topTrim}, clip]{diagrams/images/data_representation/4-pred_xy.png}
  \caption{Centroid vectors}
  \label{fig:sfig2}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.8\linewidth, trim={\leftTrim, \bottomTrim, \rightTrim, \topTrim}, clip]{diagrams/images/data_representation/4-pred_hv.png}
  \caption{Hough voting}
  \label{fig:sfig2}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.8\linewidth, trim={\leftTrim, \bottomTrim, \rightTrim, \topTrim}, clip]{diagrams/images/data_representation/4-poses.png}
  \caption{Final Pose}
  \label{fig:sfig2}
\end{subfigure}
\label{fig:dataRepresentation}

\end{figure}

==> Figures/methodology/hypothesis_pruning.tex <==

\newcommand{\leftTrim}{2.5cm}
\newcommand{\topTrim}{2cm}
\newcommand{\rightTrim}{14.5cm}
\newcommand{\bottomTrim}{10.5cm}

\includegraphics[width=\textwidth, trim={\leftTrim, \bottomTrim, \rightTrim, \topTrim}, clip]{diagrams/images/hypothesis_pruning/2-pred_hv.png}
